Statistical Inference and A/B Testing for First-Price Pacing Equilibria

We initiate the study of statistical inference and A/B testing for first-price pacing equilibria (FPPE). The FPPE model captures the dynamics resulting from large-scale first-price auction markets where buyers use pacing-based budget management. Such markets arise in the context of internet advertising, where budgets are prevalent. We propose a statistical framework for the FPPE model, in which a limit FPPE with a continuum of items models the long-run steady-state behavior of the auction platform, and an observable FPPE consisting of a finite number of items provides the data to estimate primitives of the limit FPPE, such as revenue, Nash social welfare (a fair metric of efficiency), and other parameters of interest. We develop central limit theorems and asymptotically valid confidence intervals. Furthermore, we establish the asymptotic local minimax optimality of our estimators. We then show that the theory can be used for conducting statistically valid A/B testing on auction platforms. Numerical simulations verify our central limit theorems, and empirical coverage rates for our confidence intervals agree with our theory.

==> fig/rev_coverage_pro=_0.05,_0.1,_0.2,_0.3__buyer=_10,_20,_30__item=_40,_60,_80_.tex <==
\begin{tabular}{llllllllllllll}
\toprule
   & number of buyers & \multicolumn{4}{l}{10} & \multicolumn{4}{l}{20} & \multicolumn{4}{l}{30} \\
   & beta = 1 proportion & 0.05 & 0.10 & 0.20 & 0.30 & 0.05 & 0.10 & 0.20 & 0.30 & 0.05 & 0.10 & 0.20 & 0.30 \\
number of items & value distribution &      &      &      &      &      &      &      &      &      &      &      &      \\
\midrule
\multirow{3}{*}{40} & uniform & 1.00 & 0.88 & 0.80 & 0.87 & 0.83 & 0.87 & 0.85 & 0.87 & 0.78 & 0.86 & 0.91 & 0.91 \\
   & normal & 1.00 & 0.85 & 0.85 & 0.89 & 0.86 & 0.90 & 0.89 & 0.89 & 0.82 & 0.87 & 0.93 & 0.86 \\
   & exponential & 1.00 & 0.88 & 0.90 & 0.85 & 0.79 & 0.92 & 0.90 & 0.86 & 0.81 & 0.85 & 0.86 & 0.88 \\
\cline{1-14}
\multirow{3}{*}{60} & uniform & 1.00 & 0.91 & 0.80 & 0.89 & 0.83 & 0.89 & 0.90 & 0.86 & 0.81 & 0.83 & 0.86 & 0.88 \\
   & normal & 1.00 & 0.92 & 0.89 & 0.91 & 0.87 & 0.92 & 0.82 & 0.85 & 0.93 & 0.86 & 0.89 & 0.85 \\
   & exponential & 1.00 & 0.81 & 0.90 & 0.93 & 0.85 & 0.87 & 0.93 & 0.90 & 0.92 & 0.91 & 0.86 & 0.87 \\
\cline{1-14}
\multirow{3}{*}{80} & uniform & 1.00 & 0.90 & 0.92 & 0.85 & 0.87 & 0.88 & 0.84 & 0.86 & 0.89 & 0.86 & 0.81 & 0.85 \\
   & normal & 1.00 & 0.88 & 0.87 & 0.92 & 0.92 & 0.83 & 0.90 & 0.85 & 0.85 & 0.87 & 0.89 & 0.89 \\
   & exponential & 1.00 & 0.81 & 0.84 & 0.89 & 0.87 & 0.84 & 0.93 & 0.92 & 0.85 & 0.91 & 0.92 & 0.92 \\
\bottomrule
\end{tabular}


==> fig/rev_coverage_pro=_0.05,_0.1,_0.2,_0.3__buyer=_100__item=_200_.tex <==
\begin{tabular}{llllll}
\toprule
    & number of buyers & \multicolumn{4}{l}{100} \\
    & beta = 1 proportion & 0.05 & 0.10 & 0.20 & 0.30 \\
number of items & value distribution &      &      &      &      \\
\midrule
\multirow{3}{*}{200} & uniform & 0.73 & 0.66 & 0.67 & 0.78 \\
    & normal & 0.90 & 0.81 & 0.77 & 0.82 \\
    & exponential & 0.64 & 0.76 & 0.84 & 0.84 \\
\bottomrule
\end{tabular}


==> fig/rev_coverage_table_large_scale2022-12-2718_49_18.120528.tex <==
\begin{tabular}{lllllllllll}
\toprule
    & n buyers & \multicolumn{3}{l}{10} & \multicolumn{3}{l}{20} & \multicolumn{3}{l}{30} \\
    & beta = 1 proportion &  0.2 &  0.4 &  0.5 &  0.2 &  0.4 &  0.5 &  0.2 &  0.4 &  0.5 \\
n items & value distribution &      &      &      &      &      &      &      &      &      \\
\midrule
\multirow{3}{*}{100} & uniform & 0.88 & 0.93 & 0.89 & 0.88 & 0.86 & 0.95 & 0.81 & 0.89 & 0.90 \\
    & normal & 0.89 & 0.85 & 0.90 & 0.94 & 0.84 & 0.84 & 0.90 & 0.85 & 0.88 \\
    & exponential & 0.91 & 0.85 & 0.88 & 0.90 & 0.90 & 0.90 & 0.84 & 0.93 & 0.90 \\
\cline{1-11}
\multirow{3}{*}{200} & uniform & 0.89 & 0.85 & 0.89 & 0.86 & 0.82 & 0.86 & 0.73 & 0.84 & 0.88 \\
    & normal & 0.93 & 0.95 & 0.89 & 0.84 & 0.90 & 0.87 & 0.87 & 0.89 & 0.85 \\
    & exponential & 0.89 & 0.89 & 0.90 & 0.82 & 0.82 & 0.87 & 0.88 & 0.93 & 0.84 \\
\cline{1-11}
\multirow{3}{*}{400} & uniform & 0.89 & 0.83 & 0.89 & 0.79 & 0.80 & 0.87 & 0.80 & 0.88 & 0.91 \\
    & normal & 0.86 & 0.88 & 0.90 & 0.89 & 0.90 & 0.89 & 0.88 & 0.87 & 0.87 \\
    & exponential & 0.90 & 0.97 & 0.90 & 0.88 & 0.88 & 0.85 & 0.91 & 0.89 & 0.89 \\
\bottomrule
\end{tabular}


==> markov.tex <==
\section{Extension to Markov Items}


\begin{defn}[$\beta$-mixing coefficients]
    The $\beta$-mixing coefficient between two sigma algebras $\cA_1$ and $\cA_2$ on $\Theta$ is 
    $\beta\left(\mathcal{A}_1, \mathcal{A}_2\right)=\frac{1}{2} \sup \sum_{\mathcal{I} \times \mathcal{J}}\left|\mathbb{P}\left(A_i \cap B_j\right)-\mathbb{P}\left(A_i\right) \mathbb{P}\left(B_j\right)\right|$
    where the supremum is taken over finite partitions $\{A_i\}_{i\in \mathcal{I}}$ and $\{B_j\}_{j \in \mathcal{J}}$ such that $A_i \in \cA_1$ and $B_i \in \cA_2$.
\end{defn}
For a sequence of strictly stationary random variables
$\gamma= \{\thetau\}$, given the sigma algebras $\mathcal{G}_1 \defeq \sigma\left(\theta^1 \right)$ and $\mathcal{G}_k \defeq \sigma\left(\thetau: \tau \geq k \right)$ for $k \geq 2$, the
$\beta$-mixing coefficient of the sequence $\gamma$ is $\beta_k \defeq \beta(\cG_1, \cG_{k+1})$. 
\begin{theorem}

Assume $\gamma$ is a Markov chain with an aperiodic, positive Harris recurrent Markov chain taking values on $\Theta$ with stationary distribution $\pi$.
 Then $\betagam \toprob \betast$. Moreover, 
if \nameref{as:smoothness} and \nameref{as:constraint_qualification} in the market $\FPPE(b,v, \pi)$, and the decay condition on $\beta_k$ holds:
\begin{align}
    \beta_k k ^r \to 0
\end{align} 
for some $r > 1$, then $ \sqrt t (\betagam - \betast) \tod \cN(0, \Sigma_{\beta ,\Mkv})$ and $\sqrt t (\REVgam - \REVst) \tod \cN(0, \sigma\sq_{\REV,\Mkv})$, where 
\begin{align}
    \Sigma_{\beta, \Mkv} & = \var(D_\beta(\theta^1)) + 2 \sum_{\tau = 2}^\infty \cov (D_\beta(\theta^1), D_\beta(\theta^\tau)) \notag 
    \\
    & = (\cH_B)\pinv \Omega_{\Mkv} (\cH_B) \pinv ,
    \notag
    \\
    & \text{where } \Omega_{\Mkv} = \var(\must(\theta^1)) +  2 \sumtauft \cov(\must(\theo), \must(\thet)),
    \\
    \sigma\sq_{\REV, \Mkv} & = \var(D_\REV(\theta^1)) + 2 \sum_{\tau = 2}^\infty \cov (D_\REV(\theta^1), D_\REV(\theta^\tau)) 
    .
\end{align}
\end{theorem}

\begin{proof}
By Lemma 3.1 from \citet{arcones1994central}, the condition $\beta_k k^r \to 0$ for some $r > 0$
ensures that the stochastic equicontinuity condition holds for the function classes $\cF_1$, $\cF_2$ and $\cF_1 \cdot \cF_2$, i.e.,
$\sup_{(f,g) \in [ \delta_t]_{L^2}} \nu_t (f - g) = o_p(1)$ for all $\delta_t \downarrow 0$ and $[\delta_t]_{L^2} = \{ (f,g) : f, g \in \cF, \int (f-g)\sq \diff \pi \leq \delta _t\}$ with $\cF$ being one of the three classes. 

By \todo{xxx}, the asymptotic distribution of $\betagam$ is $(\cH_B)\pinv (\frac{1}{\sqrt t}\sumtau \nabla f(\thetau, \betast))$. By a Markov CLT \todo{xx}, we have 
\begin{align}
    \frac{1}{\sqrt t}\sumtau \nabla f(\thetau, \betast) \tod \cN(0,\Omega_{\Mkv})
\end{align}
\end{proof}
\todo{add exampels, add inference procedures}
